Checking Robustness Against Snapshot Isolation

Transactional access to databases is an important abstraction allowing programmers to consider blocks of actions (transactions) as executing in isolation. The strongest consistency model is {\em serializability}, which ensures the atomicity abstraction of transactions executing over a sequentially consistent memory. Since ensuring serializability carries a significant penalty on availability, modern databases provide weaker consistency models, one of the most prominent being \emph{snapshot isolation}. In general, the correctness of a program relying on serializable transactions may be broken when using weaker models. However, certain programs may also be insensitive to consistency relaxations, i.e., all their properties holding under serializability are preserved even when they are executed over a weak consistent database and without additional synchronization. In this paper, we address the issue of verifying if a given program is {\em robust against snapshot isolation}, i.e., all its behaviors are serializable even if it is executed over a database ensuring snapshot isolation. We show that this verification problem is polynomial time reducible to a state reachability problem in transactional programs over a sequentially consistent shared memory. This reduction opens the door to the reuse of the classic verification technology for reasoning about weakly-consistent programs. In particular, we show that it can be used to derive a proof technique based on Lipton's reduction theory that allows to prove programs robust.

==> Conclusion.tex <==
%!TEX root = acmart-pacmpl-template.tex
\vspace{-3mm}
\section{Conclusion}
We have shown that the problem of verifying that a transactional program is robust against causal consistency can be reduced, using a linear-size instrumentation of the given program, to a state reachability problem in a transactional program running over a sequentially consistent shared memory. This reduction leads to the first decidability result concerning the robustness checking problem against a weak consistency model of distributed systems. Beside this, this reduction opens the door to the use of existing methods and tools for the analysis and verification of concurrent programs running over a sequentially consistent shared memory. Therefore, our result can easily be used for the design of a large spectrum of static/dynamic tools for testing/verifying robustness against causal consistency. Our approach also opens the door for the design of techniques for inserting precisely the synchronization that is needed for ensuring serializability for a specific client program. This is a topic that we leave for future work. We also think that our approach can be extended to other consistency models for distributed systems such as snapshot isolation. In fact, despite that the problem of checking robustness against snapshot isolation has been addressed in few works \cite{DBLP:conf/concur/0002G16,DBLP:journals/jacm/CeroneG18,sureshconcur2018}, its decidability and complexity issues are still open. However, such extensions are not straightforward, and their investigation is part of our future work.


